ThreeDWorld: A Platform for Interactive Multi-Modal Physical Simulation

We introduce ThreeDWorld (TDW), a platform for interactive multi-modal physical simulation. TDW enables simulation of high-fidelity sensory data and physical interactions between mobile agents and objects in rich 3D environments. Unique properties include: real-time near-photo-realistic image rendering; a library of objects and environments, and routines for their customization; generative procedures for efficiently building classes of new environments; high-fidelity audio rendering; realistic physical interactions for a variety of material types, including cloths, liquid, and deformable objects; customizable agents that embody AI agents; and support for human interactions with VR devices. TDW's API enables multiple agents to interact within a simulation and returns a range of sensor and physics data representing the state of the world. We present initial experiments enabled by TDW in emerging research directions in computer vision, machine learning, and cognitive science, including multi-modal physical scene understanding, physical dynamics predictions, multi-agent interactions, models that learn like a child, and attention studies in humans and neural networks.

==> figtext/VR.tex <==
\begin{figure*}
    \centering
    %\includegraphics[width=1.0\linewidth]{figure/fig4_larger.pdf}
    \includegraphics[width=1.0\linewidth]{figure/VR_fig_new_small.pdf}
    \caption{\tetbf{(a)} Illustration of TDW’s VR capabilities in an experiment measuring spontaneous patterns of attention to agents executing spatiotemporal kinematics typical of real-world non-animate (either static or with periodic or random motion) and animate agents. 
    %(we illustrate chasing, but other experiments include mimicry, peekaboo, and object preference). 
    By design, the stimuli are devoid of surface features, so that both humans and intrinsically-motivated neural network agents must discover which agents are interesting and thus worth paying attention to, based on the behavior of the actor agents. Example timecourses (panel \textbf{b}) and aggregate attention (panel \textbf{c}) for different agents, from humans over real time, and from intrinsically-motivated neural network agents over learning time.}
    \label{fig:VR_scene}
\end{figure*}

==> figtext/VR_result.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=1\linewidth]{figure/VR_result.png}
        \vspace{-5mm}
    \caption{Example timecourses and aggregate attention to different agents, from humans over real time (a and b), and from intrinsically-motivated neural network agents over learning time (c and d).}
    \label{fig:VR_result}
\end{figure*}

==> figtext/network.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figure/controller_build.png}
    \caption{High-level network architecture of TDW.}
    \label{fig:network}
\end{figure}

==> figtext/tdw200.tex <==
\begin{figure}[http]
   \centering
   \vspace{-5mm}
   \includegraphics[width = 0.5\linewidth]{figure/tdw200_V2.png}
    \vspace{-3mm}
   \caption{Examples from the TDW pre-training dataset, to be released as part of the TDW package.}
   \vspace{-3mm}
   \label{fig:tdw200}
\end{figure}

==> figtext/transport_fig.tex <==
\begin{figure}[http]
   \centering
   \includegraphics[width = 0.8\linewidth]{figure/top_down_task_w_annots_2021-04-06.png}
   \vspace{-2mm}

   \caption{ Embodied Agent transport task: the agent must transport objects scattered across multiple rooms and place them on the bed (marked with a green bounding box) in the bedroom. The agent can ﬁrst pick up a container, put objects into it, and then transport them to the goal location.}
   \label{fig:transport}
   \vspace{-5mm}

\end{figure}

==> table/comparison.tex <==
\begin{table*} \label{table:comparison}
	\begin{center}
	\small
		\begin{tabular}{|l|c|c|c|c|c|c|}
			 \hline
			 \multicolumn{1}{|p{0.5cm}|}{\centering Framework}
			 & \multicolumn{1}{|p{1.75cm}|}{\centering Customizable}
			 & \multicolumn{1}{|p{1.15cm}|}{\centering Photoreal \\ Scenes (I,O,C)}
			 & \multicolumn{1}{|p{1.15cm}|}{\centering Physics \\ Simulation (R,S,C,F)}
			 & \multicolumn{1}{|p{1.35cm}|}{\centering Acoustic \\ Simulation (E,P)}
			 & \multicolumn{1}{|p{1.2cm}|}{\centering Object \\ Interaction \\ (D,A,H)}\\\hline
			 \hline
			 Deepmind Lab & & & D, A\\
			 \hline
			 MuJuCo & R, C, S & & D, A\\
			 \hline
			 PyBullet & R, C, S & E & D, A\\
			 \hline
			 OpenAI Gym & & & D, A, H\\
			 \hline
			 HoME & & & R & E &  \\ 
			 \hline
			 AI2-THOR & & I & R  &  &  D \\
			 \hline
			 Gibson & & & & &  \\
			 \hline
			 Habitat & & I & & &  \\
			 \hline
			 VirtualHome & & I & & & D, A \\  
			 \hline
			 ThreeDWorld & \checkmark & I, O & R, C, S, F & E, P & D, A, H \\
			 \hline
		\end{tabular}
	\end{center}
\end{table*}





==> table/comparison_table_single_column.tex <==
\begin{table}[h]
	\begin{center}\small
		\begin{tabular}{l|c|c|c|c}
			 \hline
		 \multicolumn{1}{p{0.5cm}|}{\centering Framework}
			 & \multicolumn{1}{|p{1.0cm}|}{\centering  Scenes \\(I,O,C)}
			 & \multicolumn{1}{|p{1.15cm}|}{\centering Physics \\  (R,S,C,F)}
			 & \multicolumn{1}{|p{1.25cm}|}{\centering Acoustic \\  (E,P)}
			 & \multicolumn{1}{|p{1.2cm}}{\centering Interaction \\ (D,A,H)}\\
			 \hline
			 Deepmind Lab & & & & D, A \\
			 \hline
			 MuJuCo & & RF, C, S & & D, A \\
			 \hline
			 PyBullet & & R & & D, A \\
			 \hline
			 HoME & & R & E &  \\ 
			 \hline
			 VirtualHome & I & & & D, A \\  
			 \hline
			 Gibson & I & & &  \\
			 \hline
			 Habitat & I & & &  \\
			 \hline
			 AI2-THOR & I & R  &  &  D \\
			 \hline
			 ThreeDWorld & I, O & RF, C, S, F & E, P & D, A, H\\
			 \hline
		\end{tabular}
	\end{center}\vspace{-5mm}
		\caption{Comparison of TDW's capabilities with those of related virtual simulation frameworks.} \gc{I will redo that table.}
		\vspace{-5mm}
		\label{tab:comparison}
	\end{table}






==> table/curiosity_results.tex <==
\begin{table*}
\label{table:curiosity_results}
\caption{
\textbf{Curiosity-driven representation learning.} An agent with a curious learning policy achieves substantially higher performance on world-model prediction and visual transfer tasks then an agent implementing a random policy.  In the world-model learning tasks, the agent seeks to predict the velocity, rotation, force and torque parameters that create changes in its visual input. }

\begin{center}
\begin{small}
\begin{tabular}{lccccc}
\toprule
Task & Rand. Policy/Model & Rand. Model/Curious Policy & Learned Model/Rand. Policy & Full Model \\
\midrule
velocity prediction acc.   & 62.4 & 69.2 & 90.4 & \textbf{95.9} \\
rotation prediction acc.     & 79.0 & 80.0 & 95.5 & \textbf{98.2}\\
force prediction acc.  & 20.8 & 33.1 & 42.1 & \textbf{51.1} \\
torque prediction acc.   & 20.9 & 32.1 & 41.3 & \textbf{43.2}\\
Object frequency (\%)             & 0.50 & 47.9 & 0.40 & \textbf{61.1}  \\
\midrule
Object Presence error (\%)             & 4.0 & 3.0 & 0.92 & 0.92  \\
Localization error [px]   & 15.04 & 10.14 & 5.94 &  \textbf{4.36} \\
Recognition acc.        & 13.0 & 21.99 & 12.3 & \textbf{28.5}  \\
\midrule
Recognition acc.(2) & 12.0 & - & 16.1 & \textbf{39.7} \\
\bottomrule
\end{tabular}
\end{small}
\vspace{-3mm}
\end{center}
\end{table*} 

==> table/muli-modal.tex <==
\begin{table}[tb!]

	\begin{center}
		\begin{tabular}{l|c|c}
			Method & Material  &  Mass \\
	\hline
			Vision only & 0.72  &  0.42\\
	\hline
			Audio only & 0.92 &0.78\\
	\hline
			Vision + Audio &  \textbf{0.96} & \textbf{0.83}\\
	\hline

					\end{tabular}
		
		\caption{Comparison of the effect of physical scene understanding on material and mass classification.}
		\label{tab:multi-model}
	\end{center}


		

	\end{table}

==> table/sound_transfer.tex <==
\begin{table}[t]
	\begin{center}
		\begin{tabular}{l|c}
		\hline
			Dataset & Accuracy \\
			\hline
			Material & 82\% \\
			\hline
		\end{tabular}
	\end{center}
		\label{tab:sound}

	\caption{Sound perception transfer on material.}
	\end{table}
